Benchmarking Safe Deep Reinforcement Learning in Aquatic Navigation

We propose a novel benchmark environment for Safe Reinforcement Learning focusing on aquatic navigation. Aquatic navigation is an extremely challenging task due to the non-stationary environment and the uncertainties of the robotic platform, hence it is crucial to consider the safety aspect of the problem, by analyzing the behavior of the trained network to avoid dangerous situations (e.g., collisions). To this end, we consider a value-based and policy-gradient Deep Reinforcement Learning (DRL) and we propose a crossover-based strategy that combines gradient-based and gradient-free DRL to improve sample-efficiency. Moreover, we propose a verification strategy based on interval analysis that checks the behavior of the trained models over a set of desired properties. Our results show that the crossover-based training outperforms prior DRL approaches, while our verification allows us to quantify the number of configurations that violate the behaviors that are described by the properties. Crucially, this will serve as a benchmark for future research in this domain of applications.

==> Sections/Introduction_backup.tex <==
\section{Introduction}
\label{sec:introduction}

The applications of real-world autonomous robotic systems are driven by the development of physically realistic simulation \cite{sim_env_mujoco}, which can be difficult to design. %Such realistic simulations can be designed using the recent Unity toolkit \cite{sim_env_unity} that also incorporates an interface for external learning scripts. 

We address the lack of simulation environments for aquatic drones by presenting a novel aquatic scene characterized by a physically realistic water surface with dynamic waves. Such realistic simulations can be designed using the recent Unity toolkit \cite{sim_env_unity} that also incorporates an interface for external learning scripts. Given the variety of applications for aquatic drones \cite{aquatic_drones_intcatch, aquatic_drones_1}, exploring the autonomy of such robotic platforms is an interesting domain of applications because, for example, autonomous water quality monitoring has been already introduced as an efficient alternative to the more traditional manual sampling \cite{aquatic_drones_intcatch}.
Hence, we designed our environment to be compatible with the well-known Gym interface \cite{sim_env_gym} to promote its applicability, and we believe it is therefore an important asset to benchmark and tests future research on the autonomous capabilities of aquatic drones. 

Within such environment, we consider the robotic navigation problem to provide an initial benchmark for the aquatic navigation task. In particular,
we focus on DRL, as it attracted attention in recent literature as a solution for autonomous navigation \cite{navigation_discretedrl, navigation_drl_1} due to its ability to train decision-making policies that generalize from past experiences to adapt to unseen environments.

In more detail, we use the drones of the Horizon 2020 project INTCATCH\footnote{https://intcatch.eu/} to model the robotic platform for the simulation, aiming to train a robust policy that can autonomously navigate to random targets, avoiding collisions. Achieving complete autonomy with DRL approaches, however, present several challenges that prevent a wider utilization of such learning techniques. 

    \begin{figure}[t]
        \centering
		\includegraphics[width=0.35\textwidth]{Images/intro_sim_env.png}
      	\caption{Overall schematic of our setup.}
    \vspace{-1em}
	\end{figure}
	
%Following these issues, devising novel learning approaches to improve both the sample efficiency and the exploration, and formally guaranteeing the behavior of a trained model, are some of the main challenges 
First, DRL has to cope with the environment uncertainties, requiring a huge number of trials to achieve good performance. The lack of diverse exploration when operating in high-dimensional spaces such as our aquatic task also causes convergence to local optima. 
We address these issues by extending a recent direction that proposes the combination of gradient-free and gradient-based DRL \cite{mixed_erl, mixed_pderl, mixed_gdrl}, to assimilate the best aspects of both solutions. In more detail, %following recent works that show the effectiveness of value-based DRL (i.e., discrete action spaces) over policy-gradient (and actor-critic) solutions (i.e., continuous action spaces) \cite{navigation_discretedrl, valuebased_branching, valuebased_bigspaces}, 
we combine a crossover function, typical of Genetic Algorithms (GA), with gradient-based DRL. This allows us to improve over prior combined approaches, which are detailed in Section \ref{sec:background}. The general idea is to incorporate the sampling efficiency of gradient-based DRL while diversifying the collected experiences using the gradient-free population.

Second, robotic tasks usually involve high-cost hardware, hence the behavior of the trained policy must be evaluated to avoid potentially dangerous situations. We address the behavior analysis of these models, by extending prior formal verification \cite{verification_nips} to quantify the occurrences of dangerous situations in the input domain. We also use the state configurations where such undesirable settings occur to discuss how it is possible to exploit this information to design a controller that can avoid such unsafe behaviors.
%In detail, models that are trained for decision-making, require the analysis of multiple outputs (e.g., choose the action that maximizes a return), and prior works do not consider such relations. In contrast, they aim at directly verifying whether the bound of a single network output lies in a given interval (e.g., a motor velocity never exceeds fixed bounds).    
In more detail, we use interval analysis \cite{verification_interval_analysis} based verification to verify the relations between two or more network outputs in the case of value-based DRL (e.g., in a certain input domain, the network must not select a certain action) or the output values in the case of continuous control. In contrast to prior work that mostly considers such analysis from dependent input intervals, our approach subdivides the analysis into small input intervals that are independent of each other. This allows a straightforward parallelization and the computation of the percentage of undesirable situations, as detailed in Section \ref{sec:method_verifier}. To analyze the behavior of the trained models for aquatic navigation, we introduce a set of properties that describe core behaviors that an autonomous controller should respect in our task. This represents an initial benchmark in aquatic applications, to pave the way for future research about behavior analysis and safety.
%This enables the verification of DRL models, where the output nodes correspond to actions that are selected by the trained network, according to their value. 

Summarizing, we introduce a novel environment for aquatic drones and besides providing a benchmark for the aquatic navigation, our results highlight the following contributions: (i) the crossover-based training improves the performance (i.e., success rate) over a previous combined approach (GDRL \cite{mixed_gdrl}), as well as value-based and policy gradient DRL. Such baselines, in fact, fail at training robust policies in the same number of epochs of the proposed method. (ii) We extend a previous interval analysis tool \cite{verification_nips} to parallelize the evaluation of the properties that describe core behavior for aquatic navigation and compute a \textit{violation} metrics that quantifies the results of this analysis.

